GraphMaps: Browsing Large Graphs as Interactive Maps

Algorithms for laying out large graphs have seen significant progress in the past decade. However, browsing large graphs remains a challenge. Rendering thousands of graphical elements at once often results in a cluttered image, and navigating these elements naively can cause disorientation. To address this challenge we propose a method called GraphMaps, mimicking the browsing experience of online geographic maps. GraphMaps creates a sequence of layers, where each layer refines the previous one. During graph browsing, GraphMaps chooses the layer corresponding to the zoom level, and renders only those entities of the layer that intersect the current viewport. The result is that, regardless of the graph size, the number of entities rendered at each view does not exceed a predefined threshold, yet all graph elements can be explored by the standard zoom and pan operations. GraphMaps preprocesses a graph in such a way that during browsing, the geometry of the entities is stable, and the viewer is responsive. Our case studies indicate that GraphMaps is useful in gaining an overview of a large graph, and also in exploring a graph on a finer level of detail.

==> Makefile <==
DOC = lg
LOGFILES = $(DOC).blg $(DOC).log $(DOC).wc
DOCS = $(DOC).pdf $(DOC).ps $(DOC).dvi
LATEX = pdflatex

# FIGS=`grep '^[^%]*\/.*eps' tochi2004.tex `; FIGS=`basename $FIGS | tr ',' ' '`; echo $FIGS
#FIGSFILES = 
#FIGS = $(patsubst %,../common-figures/%,$(FIGFILES))
FIGS =

$(DOC).pdf:	$(DOC).bbl
		-taskkill /f /im acrord32.exe
		$(LATEX) $(DOC)

pdfv:	$(DOC).pdf
		-taskkill /f /im acrord32.exe
		open $(DOC).pdf &

xpdf:		$(DOC).pdf
			-taskkill /f /im acrord32.exe
			xpdf $(DOC).pdf &

pdf:		$(DOC).pdf
ps:		$(DOC).ps

$(DOC).ps:	$(DOC).pdf
		pdf2ps $(DOC).pdf $(DOC).ps

psv:		$(DOC).ps
		gv $(DOC).ps &

$(DOC).bbl:	$(DOC).aux
		bibtex $(DOC)

$(DOC).aux:	$(DOC).tex $(DOC).bib $(FIGS)
		-taskkill /f /im acrord32.exe
		$(LATEX) $(DOC)

wc:		$(DOC).wc
		echo; echo; echo "Word count:`cat $(DOC).wc | wc -w`"; echo

$(DOC).wc:      $(DOC).pdf
		ps2ascii $(DOC).pdf $(DOC).wc

clean:
		del /Q $(DOC).aux $(DOC).bbl $(LOGFILES) $(DOCS)

full: 
	-taskkill /f /im acrord32.exe
	Pdflatex $(DOC)
	Bibtex $(DOC)
	Pdflatex $(DOC)
	Pdflatex $(DOC)

